Sn 2008in - bridging the gap between normal and faint supernovae of type IIP

We present optical photometric and low-resolution spectroscopic observations of the Type II plateau supernova (SN) 2008in, which occurred in the outskirts of the nearly face-on spiral galaxy M 61. Photometric data in the X-rays, ultraviolet and near-infrared bands have been used to characterize this event. The SN field was imaged with the ROTSE-IIIb optical telescope about seven days before the explosion. This allowed us to constrain the epoch of the shock breakout to JD = 2454825.6. The duration of the plateau phase, as derived from the photometric monitoring, was ~ 98 days. The spectra of SN 2008in show a striking resemblance to those of the archetypal low-luminosity IIP SNe 1997D and 1999br. A comparison of ejecta kinematics of SN 2008in with the hydrodynamical simulations of Type IIP SNe by Dessart et al. (2010) indicates that it is a less energetic event (~ 5$\times10^{50}$ erg). However, the light curve indicates that the production of radioactive $^{56}$Ni is significantly higher than that in the low-luminosity SNe. Adopting an interstellar absorption along the SN direction of $A_V$ ~ 0.3 mag and a distance of 13.2 Mpc, we estimated a synthesized Ni mass of ~ 0.015 $M_{\odot}$. Employing semi-analytical formulae (Litvinova & Nadezhin 1985), we derived a pre-SN radius of ~ 126$R_{\odot}$, an explosion energy of ~ 5.4$\times10^{50}$ erg and a total ejected mass of ~ 16.7$M_{\odot}$. The latter indicates that the zero age main-sequence mass of the progenitor did not exceed 20$M_{\odot}$. Considering the above properties of SN 2008in, and its occurrence in a region of sub-solar metallicity ([O/H] ~ 8.44 dex), it is unlikely that fall-back of the ejecta onto a newly formed black hole occurred in SN 2008in. We therefore favor a low-energy explosion scenario of a relatively compact, moderate-mass progenitor star that generates a neutron star.

==> run <==
latex ms
latex ms
dvips -o ms.ps ms.dvi
\rm *.log
\rm *.aux
\rm *.dvi
ps2pdf ms.ps

